Active Tapping via Gaussian Process for Efficient Unknown Object Surface Reconstruction

Object surface reconstruction brings essential benefits to robot grasping, object recognition, and object manipulation. When measuring the surface distribution of an unknown object by tapping, the greatest challenge is to select tapping positions efficiently and accurately without prior knowledge of object region. Given a searching range, we propose an active exploration method, to efficiently and intelligently guide the tapping to learn the object surface without exhaustive and unnecessary off-surface tapping. We analyze the performance of our approach in modeling object surfaces within an exploration range larger than the object using a robot arm equipped with an end-of-arm tapping tool to execute tapping motions. Experimental results show that the approach successfully models the surface of unknown objects with a relative 59% improvement in the proportion of necessary taps among all taps compared with state-of-art performance.

==> papers/relatedwork.tex <==
\section{Related Work}
 A state-of-art approach in surface recognition is using tactile sensors. Compared with vision-based methods, tactile sensor is less sensitive to environmental changes such as lighting and occlusions. While tactile sensors can provide abundant information of the object, it requires expensive processing in feature selection and extraction, and noise filtering to recognize the object. Specifically, in the context of surface reconstruction, only contact positions with objects are essential to measure the surface distribution, where tactile sensor is not fully used. 
 
 
 In \cite{jia2009surface} and \cite{59353}, tactile sensors were used to obtain information about object shapes by extracting features from tactile data and project onto the object model. Such methods, however, are limited in their applicability for only being able to recognize simple shapes of object. More importantly, contact positions are not directly used to estimate the object shapes. In order to enhance the exploratory procedures on object surfaces, Allen and Michelman in \cite{59353} used central moment analysis to determine principle contact direction, and Meier \textit{et al.} in \cite{5740987} applied grid approach to build point clouds of surface points. Although those methods performed well in shape reconstruction, the time consumption cannot be neglected. 
 
 As there is a high likelihood that nearby points on a surface shares the same features, Gaussian process is used to estimate the surface function by correlations between points defined by its kernels. Standard kernels, such as Radial-basis function (RBF) kernel and Matérn kernel, compute the similarity between sample points by corresponding distance. Dragiev \textit{et al.} in \cite{5980395} and Williams and Fitzgibbon in \cite{Williams2006GaussianPI} utilized Gaussian process regression (GPR) to estimate object shapes with implicit surface representation. The regression function provides surface assessment by its mean and uncertainty of each point on the surface, which implies that the uncertainties need to be minimized with optimal posteriors fitting into the GP model. Such needs for guiding the next point to tap and measure to increase the efficiency and accuracy of surface reconstruction, are not provided in those methods. 
 
 Active learning methods are commonly studied to explore the unknown environment intelligently. Bayesian optimization, relying on probabilistic regression function and acquisition function, has been one of the most successful searching methods to find global optimal within black-box functions in minimal sampling times \cite{7759310}. Reinforcement learning, as arising approach, is also widely used to guide self-exploration based on feedback from the environment \cite{Schreiter2015SafeEF}. Yi \textit{et al.} \cite{7759723} and Björkman \textit{et al.} \cite{6696808} selected positions to touch next through highest uncertainty point in shape estimation of GPR to actively obtain the object model. The main disadvantage of these methods is that object regions need to be given as prior information to ensure the exploration happens on object surfaces. In other words, with an unknown searching space, such methods will lead to a vast of inefficient sampling at off-object spaces.  
 
 


